DeepReShape: Redesigning Neural Networks for Efficient Private Inference

Prior work on Private Inference (PI) -- inferences performed directly on encrypted input -- has focused on minimizing a network's ReLUs, which have been assumed to dominate PI latency rather than FLOPs. Recent work has shown that FLOPs for PI can no longer be ignored and incur high latency penalties. In this paper, we develop DeepReShape, a technique that optimizes neural network architectures under PI's constraints, optimizing for both ReLUs and FLOPs for the first time. The key insight is strategically allocating channels to position the network's ReLUs in order of their criticality to network accuracy, simultaneously optimizes ReLU and FLOPs efficiency. DeepReShape automates network development with an efficient process, and we call generated networks HybReNets. We evaluate DeepReShape using standard PI benchmarks and demonstrate a 2.1% accuracy gain with a 5.2$\times$ runtime improvement at iso-ReLU on CIFAR-100 and an 8.7$\times$ runtime improvement at iso-accuracy on TinyImageNet. Furthermore, we investigate the significance of network selection in prior ReLU optimizations and shed light on the key network attributes for superior PI performance.

==> figs/03figure_pareto_tiny.tex <==

%\begin{table} [t]
%\caption{Comparison with SoTA ReLU optimization methods \cite{jha2021deepreduce,cho2022selective}. Our Proposed HRNs outperform at both higher and lower ReLU counts. }
%\label{tab:SoTAvsHRN}
%\centering 
%\resizebox{0.49\textwidth}{!}{ 
%\begin{tabular}{cccc|cccc} \toprule 
%\multicolumn{4}{c}{CIFAR-100} & \multicolumn{4}{c}{TinyImageNet} \\
%\cmidrule(lr{0.5em}){1-4} 
%\cmidrule(lr{0.5em}){5-8} 
%Method & ReLUs & Acc(\%) & Lat.(s) & Method & ReLUs & Acc(\%) & Lat.(s) \\ \toprule
%SNL & 248.4K & 77.70 & 4.72 & DeepReDuce & 917.5K & 64.66 & 17.43 \\
%SNL & 180K & 77.65 & 3.42 & SNL & 512K & 64.80 & 9.73 \\
%SNL & 120K & 76.35 & 2.28 & HRN(Ours) & 847.9K & {\bf 66.71} & 16.11 \\
%HRN(Ours) & 181.2K & {\bf 79.98} & 3.44 & HRN(Ours) & 653.3K & {\bf 65.76} & 12.41 \\
%HRN(Ours) & 106.5K & {\bf 78.18} & 2.02 & HRN(Ours) & 417.8K & {\bf 65.21} & 7.94 \\ \midrule
%SNL & 15K & 67.17 & 0.29 & SNL & 59.1K & 54.40 & 1.12 \\
%HRN(Ours) & 13.3K & {\bf 67.48} & 0.25 & HRN(Ours) & 59.4K & {\bf 55.16} & 1.13 \\   \bottomrule
%\end{tabular} }
%\end{table}


\begin{figure} [htbp] \centering
%\subfloat[{\footnotesize HRNs on CIFAR-100}]{\includegraphics[width=.25\textwidth]{plots/summary_hrn_deepreduce_snl_cifar100}} 
\subfloat[ResNet34]{\includegraphics[width=.24\textwidth]{plots/relu_resnet34_deepreduce_tiny}} 
\subfloat[ResNet50]{\includegraphics[width=.24\textwidth]{plots/relu_resnet50_deepreduce_tiny}}
%\subfloat[{\footnotesize HRNs on TinyImageNet}]{\includegraphics[width=.25\textwidth]{plots/summary_hrn_deepreduce_snl_tiny}} 
\vspace{-0.8em}
\caption{HRNs vs DeepReDuce optimization on TinyImageNet}
\label{fig:ParetoTinyImageNet}
\end{figure}

 


==> figs/10figure_StageWiseReLUs.tex <==
\begin{figure} [htbp]
\centering
\subfloat[BaseCh networks]{\includegraphics[width=.33\textwidth]{plots/StageWiseReLU_R18_BaseChannelVar}} 
\subfloat[StageCh networks]{\includegraphics[width=.33\textwidth]{plots/StageWiseReLU_R18_ChMulFactVar}} 
\subfloat[HRN-5x5x3x(Proposed)]{\includegraphics[width=.33\textwidth]{plots/StageWiseReLU_HRN_2x5x3x}}\\
\subfloat[HRN-5x7x2x (Proposed)]{\includegraphics[width=.33\textwidth]{plots/StageWiseReLU_HRN_2x7x2x}} 
\subfloat[HRN-6x6x2x(Proposed)]{\includegraphics[width=.33\textwidth]{plots/StageWiseReLU_HRN_2x6x2x}} 
\subfloat[HRN-7x5x2x(Proposed)]{\includegraphics[width=.33\textwidth]{plots/StageWiseReLU_HRN_2x5x2x}}  %\vspace{-0.6em}
\caption{Impact of network's width expansion on ReLU's distribution: for ResNet18-based BaseCh (a), StageCh (b), and proposed HRN network (c). Once HRN network's ReLU align in their criticality order (at 5,5,3), the relative distribution of ReLUs remains stable with increasing $\alpha$ values.} 
\label{fig:StageWiseReLU}
\end{figure} 

%\begin{figure} [htbp]
%\centering
%\subfloat[HRN-5x7x2x (Proposed)]{\includegraphics[width=.33\textwidth]{plots/StageWiseReLU_HRN_2x7x2x}} 
%\subfloat[HRN-6x6x2x(Proposed)]{\includegraphics[width=.33\textwidth]{plots/StageWiseReLU_HRN_2x6x2x}} 
%\subfloat[HRN-7x5x2x(Proposed)]{\includegraphics[width=.33\textwidth]{plots/StageWiseReLU_HRN_2x5x2x}} 
%\caption{ReLU distribution analysis in HRN networks by progressively increasing the $\alpha$ values from $\alpha$=2, enabling a comprehensive characterization of ReLU distribution. Once the network's achieve ReLU equalization {--} (5, 7, 2) for HRN-5x7x2x, (6, 6, 2) for HRN-6x6x2x, and (7, 5, 2) for HRN-7x5x2x {--} the (relative) ReLU distribution remains stable with increasing $\alpha$ value. }
%\label{fig:AppendixStageWiseReLUs}
%\end{figure} 

%Effect on the (relative) distribution of ReLUs when network's width is augmented by: (a) increasing the base channel count; (b) increasing the stagewise channel multiplication factors; ((c)-(f))  proposed HRN networks. The baseline network here is ResNet18 with base channel count $m$=16. {\bf Unlike StageCh networks,  the relative distribution of ReLUs in HRN networks remain unchanged at higher values of $\alpha$}.}


%Values of $\alpha$ in HRN is swept for a holistic characterization.

%\begin{wrapfigure}{5}{0.7\textwidth}
%\centering
%\subfloat[BaseCh networks]{\includegraphics[scale=0.11]{plots/StageWiseReLU_R18_BaseChannelVar}} 
%\subfloat[StageCh networks]{\includegraphics[scale=0.09]{plots/StageWiseReLU_R18_ChMulFactVar}} 
%\subfloat[(Proposed) HRN]{\includegraphics[scale=0.09]{plots/StageWiseReLU_HRN_2x5x3x}} \vspace{-0.6em}
%\caption{Network ReLUs' distribution for ResNet18-based $BaseCh$ (a), $StageCh$, and proposed criticality-aware HRN networks (c). Once HRN network achieves ReLU equalization, increasing $\alpha$ does not change the relative distribution of ReLUs across stages.} 
%\label{fig:StageWiseReLU}
%\vspace{-1em}
%\end{wrapfigure}

%with $\alpha\geq2$  and ($\beta$, $\gamma$) = (5,3)




==> figs/28figure_HRN_flops_relu_comp.tex <==

\begin{figure*} [t]
\centering
\subfloat[ReLU-efficiency: HRNs]{\includegraphics[width=.25\textwidth]{plots/relus_resnet18_vs_hrn_cifar100}}
\subfloat[ReLU-efficiency: RegNet-X]{\includegraphics[width=.25\textwidth]{plots/relus_regnetx_vs_hrn_cifar100}} 
\subfloat[ReLU-efficiency: ResNet34]{\includegraphics[width=.25\textwidth]{plots/relus_resnet34_vs_hrn_tiny}}
\subfloat[ReLU-efficiency: ResNet50]{\includegraphics[width=.25\textwidth]{plots/relus_resnet50_vs_hrn_tiny}} \\ 
\subfloat[FLOPs-efficiency: HRNs]{\includegraphics[width=.25\textwidth]{plots/flops_resnet18_vs_hrn_cifar100}} 
\subfloat[FLOPs-efficiency: RegNet-X]{\includegraphics[width=.25\textwidth]{plots/flops_regnetx_vs_hrn_cifar100}} 
\subfloat[FLOPs-efficiency: ResNet34]{\includegraphics[width=.25\textwidth]{plots/flops_resnet34_vs_hrn_tiny}}
\subfloat[FLOPs-efficiency: ResNet50]{\includegraphics[width=.25\textwidth]{plots/flops_resnet50_vs_hrn_tiny}} \\
\subfloat[HRN-5x7x2x]{\includegraphics[width=.25\textwidth]{plots/StageWiseReLU_HRN_2x7x2x}} 
\subfloat[RegNet-X]{\includegraphics[width=.25\textwidth]{plots/StageWiseReLU_RegNetX_cifar100}}
\subfloat[ResNet34: ConvNeXt \& HRNs]{\includegraphics[width=.25\textwidth]{plots/StageWiseReLU_ResNet34_cifar100}}
\subfloat[ResNet50: ConvNeXt \& HRNs]{\includegraphics[width=.25\textwidth]{plots/StageWiseReLU_ResNet50_cifar100}} \vspace{-0.8em}
\caption{FLOPs-ReLU-Accuracy tradeoff along with their stagewise ReLUs' distribution in proposed HybReNet(HRN), and their comparison with SoTA network design methods RegNet and ConvNeXt (CNeXt). {\em HRNs surpass the ReLU-efficiency of $StageCh$ models, while using fewer FLOPs}, and achieve FLOPs-ReLU-Accuracy balance (a,e). Moreover,  networks designed by SoTA design methods, RegNet-X (b,f) and  ConvNeXt-ify ResNet34/ResNet50 (c,g)/(g,h) {\em are inferior to their HRNs}, for FLOPs-ReLU-Accuracy tradeoffs. }
\label{fig:FlopsReluCompHRN}
\end{figure*} 




==> figs/32figure_NoCulling_DeepReShape.tex <==
\begin{figure} [t]
\centering
\subfloat[ResNet18Ch16]{\includegraphics[width=.25\textwidth]{plots/Re2VsScaling_ResNet18Ch16_2x2x2x_cifar100}}
\subfloat[ResNet18Ch32]{\includegraphics[width=.25\textwidth]{plots/Re2VsScaling_ResNet18Ch32_2x2x2x_cifar100}}
\subfloat[ResNet18Ch64]{\includegraphics[width=.25\textwidth]{plots/Re2VsScaling_ResNet18Ch64_2x2x2x_cifar100}}
\subfloat[ResNet18Ch128]{\includegraphics[width=.25\textwidth]{plots/Re2VsScaling_ResNet18Ch128_2x2x2x_cifar100}} \\
\subfloat[4x4x4x]{\includegraphics[width=.25\textwidth]{plots/Re2VsScaling_ResNet18Ch16_4x4x4x_cifar100}}
\subfloat[2x6x2x]{\includegraphics[width=.25\textwidth]{plots/Re2VsScaling_ResNet18Ch16_2x6x2x_cifar100}}
\subfloat[5x5x3x]{\includegraphics[width=.25\textwidth]{plots/Re2VsScaling_ResNet18Ch16_5x5x3x_cifar100}}
\subfloat[6x6x2x]{\includegraphics[width=.25\textwidth]{plots/Re2VsScaling_ResNet18Ch16_6x6x2x_cifar100}} \\
\caption{DeepReShape without Culling}
\label{fig:NoCullingDeepReShape}
\end{figure} 


==> figs/39figure_AlphaVar_HRN.tex <==
\begin{figure} [t]
\centering
\subfloat[HRN-2x5x2x]{\includegraphics[width=.25\textwidth]{plots/AlphaVar_HRN_2x5x2x_cifar}}
\subfloat[HRN-2x5x3x]{\includegraphics[width=.25\textwidth]{plots/AlphaVar_HRN_2x5x3x_cifar}}
\subfloat[HRN-2x6x2x]{\includegraphics[width=.25\textwidth]{plots/AlphaVar_HRN_2x6x2x_cifar}}
\subfloat[HRN-2x7x2x]{\includegraphics[width=.25\textwidth]{plots/AlphaVar_HRN_2x7x2x_cifar}} \\
\caption{Effect of increasing $\alpha$ (the channel multiplication factor in Stage2) for baseline networks (from left to right) HRN-2x5x2x, HRN-2x5x3x, HRN-2x6x2x, and HRN-2x7x2x: The ReLU-efficiency of networks with higher $\alpha$ does not improve, in fact it significantly reduces at lower ReLU count. }
\label{fig:AlphaVarWithCulling}
\end{figure} 


==> figs/42figure_relu_reuse_vs_snl.tex <==

\begin{figure} [t]
\centering
%\subfloat[HRN-2x5x3x]{\includegraphics[width=.33\textwidth]{plots/hybrenet_relu_2x5x3x_cifar100}}
%\subfloat[HRN-2x5x2x]{\includegraphics[width=.33\textwidth]{plots/hybrenet_relu_2x5x2x_cifar100}} 
%\subfloat[HRN-2x6x2x]{\includegraphics[width=.33\textwidth]{plots/hybrenet_relu_2x6x2x_cifar100}} \\
\subfloat[HRN-2x7x2x]{\includegraphics[width=.25\textwidth]{plots/hybrenet_relu_2x7x2x_cifar100}}
\subfloat[HRN-2x9x2x]{\includegraphics[width=.25\textwidth]{plots/hybrenet_relu_2x9x2x_cifar100}}
%\subfloat[HRN-2x6x3x]{\includegraphics[width=.33\textwidth]{plots/hybrenet_relu_2x6x3x_cifar100}}
\vspace{-0.8em}
\caption{ReLU-reuse (Re2) vs SNL on CIFAR-100. Algorithm \ref{algo:DeepReDuceAndReLUReuse} is used for the accuracy points on Pareto frontier, and the results with conventional scaling methods is represented as ``w/o Re2".  }
\label{fig:ReluReuseVsSNL}
\end{figure} 



%\caption{Experimental results for ReLU-reuse on CIFAR-100. We plot  channelwise SNL, an unstructured ReLU dropping, for fair comparison with our proposed ReLU-reuse (denoted as Re2), a structured ReLU dropping. We note that with ReLU-reuse {\bf a gain of 1\% - 3\% accuracy at iso-ReLU} has been achieved (on CIFAR-100). Compared to channel-wise SNL, HRNs achieves a substantial gain in accuracy on all the ReLU counts.}

==> figs/45figure_sensitivity_analysis.tex <==


%\begin{figure}[htbp] \centering
%\includegraphics[scale=0.3]{plots/relu_reuse} 
%\caption{Proposed ReLU-reuse where ReLUs are {\em selectively} used in a fraction of channels, reducing network's ReLUs upto 16$\times$.} 
%\label{fig:ReLUreuse}
%\end{figure}


\begin{wrapfigure}[10]{r}{0.45\textwidth}
\centering
\subfloat[ReLU efficiency]{\includegraphics[width=.23\textwidth]{plots/sensitivity_analysis_relu_cifar100}}
\subfloat[FLOPs efficiency]{\includegraphics[width=.23\textwidth]{plots/sensitivity_analysis_flops_cifar100}} \vspace{-0.6em}
\caption{Sensitivity analysis  for ReLUs and FLOPs efficiency (ResNet18 on CIFAR-100).} 
\label{fig:SensitivityAnalysis}

\end{wrapfigure}



==> tables/layerwise_flops_relu.tex <==

\def\cellheight{0.3cm}

\begin{table} [t] \centering 
\caption{Layerwise trends  of FLOPs and ReLUs (from initial to deeper layers)  when network's width is increases by (homogeneously)augmenting $\alpha$,$\beta$, and $\gamma$. {\em Distinct homogeneous} sets of ($\alpha$,  $\beta$, $\gamma$) are required for FLOPs and ReLU efficiency.} 
\label{tab:LayerwiseFLOPsReLUs}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{ccccc} \toprule
& ($\alpha, \beta, \gamma$)=2 & 2$<$($\alpha, \beta, \gamma$)$<$4 & ($\alpha, \beta, \gamma$)=$4$ & ($\alpha, \beta, \gamma$)$>$4 \\ \toprule 
Layerwise FLOPs &constant & increasing ($\uparrow$)& increasing ($\uparrow\uparrow$)& increasing ($\uparrow\uparrow\uparrow$)\\ [\cellheight]
Layerwise ReLUs & decreasing ($\downarrow\downarrow$)& decreasing ($\downarrow$) & constant & increasing ($\uparrow$) \\ \bottomrule
\end{tabular}}
\end{table}

